Automatic Segmentation of the Optic Nerve Head Region in Optical Coherence Tomography: A Methodological Review

The optic nerve head represents the intraocular section of the optic nerve (ONH), which is prone to damage by intraocular pressure. The advent of optical coherence tomography (OCT) has enabled the evaluation of novel optic nerve head parameters, namely the depth and curvature of the lamina cribrosa (LC). Together with the Bruch's membrane opening minimum-rim-width, these seem to be promising optic nerve head parameters for diagnosis and monitoring of retinal diseases such as glaucoma. Nonetheless, these optical coherence tomography derived biomarkers are mostly extracted through manual segmentation, which is time-consuming and prone to bias, thus limiting their usability in clinical practice. The automatic segmentation of optic nerve head in OCT scans could further improve the current clinical management of glaucoma and other diseases. This review summarizes the current state-of-the-art in automatic segmentation of the ONH in OCT. PubMed and Scopus were used to perform a systematic review. Additional works from other databases (IEEE, Google Scholar and ARVO IOVS) were also included, resulting in a total of 27 reviewed studies. For each algorithm, the methods, the size and type of dataset used for validation, and the respective results were carefully analyzed. The results show that deep learning-based algorithms provide the highest accuracy, sensitivity and specificity for segmenting the different structures of the ONH including the LC. However, a lack of consensus regarding the definition of segmented regions, extracted parameters and validation approaches has been observed, highlighting the importance and need of standardized methodologies for ONH segmentation.

==> LC OCT segmentation (arxiv)/Results_Table.tex <==
\def\arraystretch{1.5}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}

\begin{scriptsize}
\begin{landscape}
%\begin{table*}
\begin{longtable}{C{2cm}C{3cm}C{3.5cm}C{15cm}}
\caption{Results}\\ \hline
%\begin{tabular}{p{20mm}p{30mm}p{35mm}p{150mm}}

%\hline

Segmentation            & Outcome              & Metrics & Results \\ \hline
\multirow{5}{*}{Boundary based}  & \ac{BMO} 
& (i) Correlation with ground truth; 
(ii) Error compared with ground truth; 
(iii) Mean unsigned error; 
(iv) Mean signed error;
(v) Dice similarity coefficient;
(vi) Failure rate;
(vii) Mean average precision
&    
(i) 0.93 \citep{Boyer2006}; 
(ii) 32.03 $\pm$ 58.68 $\mu$m \citep{Mokhtari2017}. 12.4 $\pm$ 12.1 pixels \citep{Fu2015}. 2.8 pixels (normal) and 3.1 pixels (glaucoma) \citep{Paul2015}. 54.18 $\pm$ 53.74 $\mu$m \citep{Hussain2015}. 60.00 $\pm$ 42.00 $\mu$m \citep{Wu2015}. 49.28 $\pm$ 16.78 $\mu$m \citep{Miri2017}. 42.38 $\pm$ 18.33 $\mu$m \citep{Chen2019}.
(iii) 61.86 $\pm$ 61.97 $\mu$m (x axis) and 12.40 $\pm$ 11.24 $\mu$m (z axis) \citep{Yadav2018}. 49.53 $\pm$ 30.41 $\mu$m (x axis) and 31.58 $\pm$ 21.06 $\mu$m (z axis) \citep{Antony2014}. 37.98 $\pm$ 14.91 $\mu$m (x axis) and 22.28 $\pm$ 8.58 $\mu$m (z axis) \citep{Miri2017}. 9.80 $\pm$ 31.90 $\mu$m \citep{Skander2020}. 0.023 mm \citep{Lee2009}. 0.026 mm \citep{Lee2010}
(iv)  −7.69 $\pm$ 87.27 $\mu$m (x axis) and −1.41 $\pm$ 16.69 $\mu$m (z axis) \citep{Yadav2018}. 26.49 $\pm$ 40.22 $\mu$m (x axis) and 25.45 $m$ 14.37 $\mu$m (z axis) \citep{Antony2014}. -9.49 $\pm$ 24.58 $\mu$m (x axis) and 8.33 $\pm$ 17.72 $\mu$m (z axis) \citep{Miri2017}.
(v) 0.925 $\pm$ 0.030 \citep{Yu2018}. 0.959 $\pm$ 0.032 \citep{Skander2020}. 0.65 $\pm$ 0.14 \citep{Lee2010}.
(vi) 0 in 92.5\% of the scans \citep{Belghith2014}
(vii) 0.8547 for glaucoma and 0.9567 for control subjects \citep{Heisler2020}.
\\ \cline{2-4} 
                                & \ac{BMO-MRW}              
&  (i) Mean unsigned error;
(ii) Mean signed error; 
(iii) RMSE
&  (i) 58.62 $\pm$ 43.12 $\mu$m \citep{Hussain2015}. 26.65 $\pm$ 13.27 $\mu$m \citep{Antony2014}. 22.22 $\pm$ 5.99 $\mu$m \citep{Miri2017}.
(ii) 6.61 $\pm$ 18.59 $\mu$m \citep{Antony2014}. -0.30 $\pm$ 12.44 $\mu$m \citep{Miri2017}.
(iii) 17.99 $\pm$ 8.15 $\mu$m \citep{Antony2014}. 11.62 $\pm$ 4.63 $\mu$m \citep{Miri2017} \\ \cline{2-4} 
                                & Optic cup            
&  (i) Correlation with ground truth;   
(ii) Error compared with ground truth;
(iii) Mean unsigned error;
(iv) Dice similarity coefficient
&  (i) 0.80 \citep{Boyer2006}
(ii) 3.4 pixels (normal) and 3.6 pixels (glaucoma) \citep{Paul2015}
(iii) 0.009 mm \citep{Lee2009}. 0.038 mm \citep{Lee2010}
(iv) 0.85 $\pm$ 0.06 \citep{Lee2010} \\ \cline{2-4} 
                                & \ac{CDR}  
& (i) Error compared with ground truth;
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
& (i) 0.045 $\pm$ 0.033 \citep{Wu2015} 
(ii) 86.2 $\pm$ 7.1\% \citep{Khalil2018}
(iii) 86.2 $\pm$ 9.8\% \citep{Khalil2018}
(iv) 85.5 $\pm$ 5.2\% \citep{Khalil2018} \\ \cline{2-4} 
                                & \ac{ILM}   
&  (i) Mean unsigned error; 
(ii) Mean Dice coefficient;
(iii) Error compared with ground truth;
(iv) Mean Euclidean distance error
&   (i) 5.38 $\pm$ 4.23 $\mu$m \citep{Yu2018}.
(ii) 0.97 \citep{Heisler2020}.
(iii) 4.80 $\mu$m \citep{Gawlik2018}
(iv) 7.08 $\pm$ 3.7 pixels \citep{Ramzan2018a}. 7.03 $\pm$ 3.72 pixels \citep{Ramzan2018b} \\ \cline{2-4} 
                                & \ac{LC}                   
&  (i) Failure rate;  
(ii) Accuracy
&  (i) 0 in 73.7\% of the scans \citep{Belghith2015} 
(ii) 90.6\% \citep{Mao2019}      \\ \cline{2-4} 
                                & \ac{ONH} surface depth                
&   (i) Error compared with ground truth     
&    (i)  0.7 $\pm$ 1.0 \% \citep{Ko2016}.   \\ \hline
\multirow{6}{*}{Region based}   & \ac{RNFL} + prelamina     
& (i) Dice coefficient;
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
& (i) 0.82 $\pm$ 0.05 \citep{Devalla2018a}. 0.92 $\pm$ 0.05 for healthy and 0.92 $\pm$ 0.03 for glaucoma \citep{Devalla2018}. 
(ii) 0.89 $\pm$ 0.04 \citep{Devalla2018a}
(iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.
(iv) 0.93 $\pm$ 0.02 \citep{Devalla2018a} \\ \cline{2-4} 
                                & \ac{RPE}                  
& (i) Dice coefficient 
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
& (i) 0.84 $\pm$ 0.02  \citep{Devalla2018a}. 0.83 $\pm$ 0.04 for healthy and 0.84 $\pm$ 0.03 for glaucoma \citep{Devalla2018}.
(ii) 0.90 $\pm$ 0.03 \citep{Devalla2018a}
(iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.
(iv) 0.93 $\pm$ 0.02 \citep{Devalla2018a}
 \\ \cline{2-4} 
                                & Other retinal layers 
& (i) Dice coefficient
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
&  (i) 0.86 $\pm$ 0.03  \citep{Devalla2018a}. 0.95 $\pm$ 0.01 for healthy and 0.96 $\pm$ 0.03 for glaucoma \citep{Devalla2018}.
(ii) 0.98 $\pm$ 0.02 \citep{Devalla2018a}
(iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.
(iv) 0.98 $\pm$ 0.01 \citep{Devalla2018a}
 \\ \cline{2-4} 
                                & Choroid              
& (i) Dice coefficient
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
&  (i) 0.85 $\pm$ 0.02 \citep{Devalla2018a}. 0.90 $\pm$ 0.03 for healthy and 0.91 $\pm$ 0.05 for glaucoma \citep{Devalla2018}.
(ii) 0.91 $\pm$ 0.02 \citep{Devalla2018a}
(iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.
(iv) 0.93 $\pm$ 0.01 \citep{Devalla2018a}        \\ \hline 

\label{tab:results}
%\end{tabular}
\end{longtable}
%\end{table*}
\end{landscape}
\end{scriptsize}

==> LC OCT segmentation (arxiv)/Summary_Table.tex <==
\def\arraystretch{1.5}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\begin{scriptsize}
\begin{landscape}
\begin{longtable}{C{1.8cm}C{1.5cm}C{3cm}C{3.5cm}C{4.5cm}C{4.5cm}C{1cm}C{2.5cm}}
\caption{Characteristics of the reviewed studies}\\ \hline
\textbf{Category} &
  \textbf{Authors} &
  \textbf{Dataset} &
  \textbf{Regions Segmented} &
  \textbf{Validation} &
  \textbf{Results} &
  \textbf{Technique} &
  \textbf{Device} \\ \hline
\endhead

  Conventional &
  \citet{Boyer2006} &
  59 glaucoma B-scans  &
  Retinal-vitreal boundary, limits of the \ac{OD}, retinal-choroid boundaries. &
  Comparison with the ground truth. &
  High correlation between automatic and manual cup and disk limits. &
  - &
  OCT 3000 from Zeiss-Humphrey \\ \hline 

  Conventional &
  \citet{Hussain2015} &
 13 glaucoma scans &
  ILM, BMO, HRC, RNFL, RPE, \ac{OD} boundary &
  Comparison with ground truth and existing method. Confusion matrix based metrics. Distance metrics.&
  Robust segmentation over noise and pathology.&
  SD-OCT &
  Spectralis \\ \hline  
 
  Conventional &
  \citet{Belghith2015} &
  50 healthy scans and 50 glaucoma scans &
  LC anterior surface &
  Comparison with ground truth.  Statistical tests. &
  High similarity between manual and automatic segmentation. Significant correlation between changes in IOP and the position of the LC. &
  EDI SD-OCT &
  Spectralis \\ \hline   

  Conventional &
  \citet{Ko2016} &
  no info &
  ILM, BMO &
  Comparison with ground truth.  &
  Accurate segmentation of the ONH structure. Not sensitive to the differentiation of blood vessels from the ONH surface. &
  SD-OCT &
  Spectralis \\ \hline  

 Conventional &
  \citet{Mokhtari2017} &
  40 healthy scans &
  RPE break points, RPE boundary &
  Comparison with ground truth. &
  Accurate segmentation of the \ac{OD} boundary. &
  no info &
  Topcon model of 3D-1000 unit \\ \hline   

Conventional &
  \citet{Gawlik2018} &
  71 healthy scans and 345 pathological scans (31 IIH + 60 NMOSD + 252 MS) &
  ILM &
  Statistical tests. Comparison with segmentation from a device. Distance metrics. Visual evaluation.&
  Robust segmentations over variations in ONH topology. Outperforms device segmentation.&
  SD-OCT &
  Spectralis \\ \hline  

Conventional &
  \citet{Khalil2018} &
  22 healthy scans and 28 glaucoma scans  &
  ILM and RPE &
  Comparison with ground truth. Comparison with computed generated values. Comparison with existing methods \citet{wang2013quantitative, nithya2015analysis, babu2015optic}.&
  Outperforms existing methods and computer generated values.&
  SD-OCT &
  no info \\ \hline  
 
 Conventional &
  \citet{Yadav2018} &
  71 healthy scans and 177  pathological scans (31 IIH +146 autoimmune central nervous system disorders ) &
  RPE, BMO Points, ILM and BMO. &
  Comparison with ground truth. Distance metrics. &
  Successfully captures the differences between pathological groups.&
  SD-OCT &
  Spectralis \\ \hline
  
  Conventional &
  \citet{Ramzan2018a} &
  50 scans from healthy and glaucoma patients &
  ILM and RPE &
  Comparison with ground truth. comparison with computer generated values. Confusion matrix based metrics.&
  High correlation with ground truth. Outperforms existing techniques.&
  TOPCON'S 3D OCT-1000 \\ \hline 
 
 Conventional &
  \citet{Ramzan2018b} &
  50 scans from healthy and glaucoma patients &
  ILM &
  Comparison with ground truth. Distance metrics. Visual evaluation. &
  Accurate segmentation. &
  SD-OCT &
  Topcon \\ \hline 
 
 Conventional &
  \citet{Syga2019} &
  86 healthy scans and 169 glaucoma scans &
  ILM, BM points and LC &
  Statistical tests. Confusion matrix based metrics. &
  Statiscally significant differences between glaucoma patients (POAG and GODA) and healthy controls. The mean LC shapes for POAG and GODA were not significantly different.&
  EDI OCT &
  Spectralis \\ \hline 
  
Conventional &
  \citet{Mao2019} &
  72 glaucoma scans &
  LC anterior surface &
  Comparison with ground truth. Visual evaluation.&
  Segmentation accuracy is significantly higher when a deep learning noise reduction algorithm is used than in raw images.&
  SS-OCT &
  Topcon \\ \hline
 
 Machine learning &
  \citet{Lee2009} &
  30 glaucoma scans  &
  3 intraretinal surfaces, \ac{OD} boundary &
  Comparison with ground truth. Distance metrics. &
  No signifficant differences between the unsigned errors of the optic cup and disk, before and after feature selection. &
  HD-OCT &
  Cirrus \\ \hline
  
  Machine learning &
  \citet{Lee2010} &
  27 glaucoma scans &
  4 intraretinal surfaces, \ac{OD} boundary &
  Comparison with the ground truth. Distance metrics. Confusion matrix based metrics. &
  Contextual 9-k-NN outperforms the regular k-NN classifier when no post processing is applied. Performance of 9-k-NN classifier is significantly better with post processing.&
  HD-OCT &
  Cirrus \\ \hline 
 
  Machine learning &
  \citet{Antony2014} &
  44 glaucoma scans  &
  BM, intraretinal surfaces, ONH hole &
  Comparison with ground truth and existing methods. Distance metrics. Confusion matrix based metrics.&
  Outperforms existing methods \citet{hu2010automated, Lee2010}. &
  SD-OCT &
  Cirrus \\ \hline
 
  Machine learning &
  \citet{Wu2015} &
  42 glaucoma scans  &
  ILM, RPE &
  Comparison with ground truth and existing method. Distance metrics. Confusion matrix based metrics. &
  Outperforms existing methods \citet{Lee2010}. &
  SD-OCT &
  Cirrus \\ \hline
 
  Machine learning &
  \citet{Fu2015} &
  48 healthy scans  &
  ILM, RPE, \ac{OD} boundary &
  Comparison with ground truth and other methods.  &
  Outperforms existing methods \citet{Boyer2006}. &
  SD-OCT &
  Topcon \\ \hline 
 
  Machine learning &
  \citet{Paul2015} &
  25 glaucoma B-scans &
  Retinal layers, \ac{OD} boundary &
  Comparison with ground truth. &
  Correct segmentation in normal and glaucoma affected images.&
  no info &
  no info \\ \hline
 
  Machine learning &
  \citet{Miri2017} &
  69 glaucoma scans &
  ILM, (IS/OS), BM &
  Comparison with ground truth and existing methods. Distance metrics. Statistical tests. &
  Outperforms existing methods \citet{Antony2014}. &
  HD-OCT &
  Cirrus \\ \hline

   Machine learning &
  \citet{Yu2018} &
  30 healthy scans and 35 glaucoma scans &
  RNFL, retinal layers, RPE/Bruch’s complex and \ac{OD} boundary &
  Comparison with ground truth and existing methods. Confusion matrix based metrics. Distance metrics.&
  Outperforms existing methods \cite{Hu2009, zang2017automated}. &
  SD-OCT &
  Topcon \\ \hline
 
 Deep learning &
  \citet{Belghith2014} &
  100 healthy scans and 105 glaucoma scans &
  BM &
  Comparison with ground truth, values from the device and other methods. Statistical tests.&
  High correlation with ground truth and built-in software of the device. Significant differences between glaucoma and healthy eyes.&
  EDI SD-OCT &
  Cirrus and Spectralis \\ \hline 
 
 Deep learning &
  \citet{Devalla2018a} &
  40 healthy scans and 60 glaucoma scans &
  RNFL and the prelamina; RPE; all other retinal layers; the choroid; the peripapillary sclera and the LC; &
  Confusion matrix based metrics. Statistical tests.&
  Good performance for all tissues in glaucoma and healthy images. Performs better with compensated images.&
  EDI SD-OCT &
  Spectralis \\ \hline
 
 Deep learning &
  \citet{Devalla2018} &
  40 healthy scans and 60 glaucoma scans &
  RNFL and the prelamina; RPE; all other retinal layers; choroid; peripapillary sclera; LC; &
  Confusion matrix based metrics. &
  Good performance for all tissues in glaucoma and healthy images. No significant differences in segmentation performances with compensated and uncompensated images.&
  EDI OCT &
  Spectralis \\ \hline
 
 Deep learning &
  \citet{Chen2019} &
  30 glaucoma scans &
  \ac{OD} boundary, RPE, BMO points &
  Comparison with the ground truth and with existing methods.&
  Outperforms existing methods \cite{Hussain2015, Wu2015, Miri2017}. &
  SD-OCT &
  Topcon \\ \hline
 
 Deep learning &
  \citet{Heisler2020} &
  42 healthy scans and 80 glaucoma scans &
  ILM, RNFL, BM, choroid-sclera boundary; BMO points &
  Comparison with ground truth. Confusion matrix based metrics. Statistical tests. &
  No statistically significant difference between BMO segmentation and ground truth. Thickness parameters were highly correlated.&
  SS-OCT &
  custom-built OCT \\ \hline
 
 Deep learning &
  \citet{Devalla2020} &
  225 healthy scans and 225 glaucoma scans &
  RNFL and prelamina; ganglion cell complex; all other retinal layers; RPE; choroid; LC &
  Confusion matrix based metrics. Visual evaluation. Statistical tests. &
  Networks trained in any of the devices, successfully segmented images from other devices with high performances in all tissues.&
  SD-OCT &
  Spectralis, Cirrus and RTVue \\ \hline

  Deep learning &
\citet{Skander2020} &
  102 healthy scans and 223 glaucoma scans &
  BMO &
  Comparison with ground truth. Confusion matrix based metrics. Distance metrics.&
  U-net like architecture with B-scans as input had the best performance.&
  SD-OCT &
  Spectralis \\ \hline

\end{longtable}
\end{landscape}
\end{scriptsize}

==> LC OCT segmentation (arxiv)/boundary_based.tex <==
\begin{table*}[h]
\centering
\caption{Results from the boundary based segmentations.}
\label{tab:boundary based}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lll}
\hline
%\multicolumn{3}{c}{Boundary based segmentation} \\ \hline
\multicolumn{1}{c}{Outcome} &
  \multicolumn{1}{c}{Metrics} &
  \multicolumn{1}{c}{Results} \\ \hline
BMO &
  \begin{tabular}[c]{@{}l@{}}(i) Correlation with ground truth; \\ \\ (ii) Error compared with ground truth; \\ \\ (iii) Mean unsigned error; \\ \\ (iv) Mean signed error;\\ \\ (v) Dice similarity coefficient;\\ \\ (vi) Failure rate;\\ \\ (vii) Mean average precision\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 0.93 \citep{Boyer2006}; \\ (ii) 32.03 $\pm$ 58.68 $\mu$m \citep{Mokhtari2017}. 12.4 $\pm$ 12.1 pixels \citep{Fu2015}. \\ 2.8 pixels (normal) and 3.1 pixels (glaucoma) \citep{Paul2015}. \\ 54.18 $\pm$ 53.74 $\mu$m \citep{Hussain2015}. \\ 60.00 $\pm$ 42.00 $\mu$m \citep{Wu2015}. 49.28 $\pm$ 16.78 $\mu$m \citep{Miri2017}. \\ 42.38 $\pm$ 18.33 $\mu$m \citep{Chen2019}.\\ (iii) 61.86 $\pm$ 61.97 $\mu$m (x axis) and 12.40 $\pm$ 11.24 $\mu$m (z axis) \citep{Yadav2018}. \\ 49.53 $\pm$ 30.41 $\mu$m (x axis) and 31.58 $\pm$ 21.06 $\mu$m (z axis) \citep{Antony2014}. \\ 37.98 $\pm$ 14.91 $\mu$m (x axis) and 22.28 $\pm$ 8.58 $\mu$m (z axis) \citep{Miri2017}. \\ 9.80 $\pm$ 31.90 $\mu$m \citep{Skander2020}. \\ 0.023 mm \citep{Lee2009}. 0.026 mm \citep{Lee2010}\\ (iv)  -7.69 $\pm$ 87.27 $\mu$m (x axis) and -1.41 $\pm$ 16.69 $\mu$m (z axis) \citep{Yadav2018}. \\ 26.49 $\pm$ 40.22 $\mu$m (x axis) and 25.45 $m$ 14.37 $\mu$m (z axis) \citep{Antony2014}.\\  -9.49 $\pm$ 24.58 $\mu$m (x axis) and 8.33 $\pm$ 17.72 $\mu$m (z axis) \citep{Miri2017}.\\ (v) 0.925 $\pm$ 0.030 \citep{Yu2018}. 0.959 $\pm$ 0.032 \citep{Skander2020}. \\ 0.65 $\pm$ 0.14 \citep{Lee2010}.\\ (vi) 0 in 92.5\% of the scans \citep{Belghith2014}\\ (vii) 0.8547 for glaucoma and 0.9567 for control subjects \citep{Heisler2020}.\end{tabular} \\ \hline
BMO-MRW &
  \begin{tabular}[c]{@{}l@{}}(i) Mean unsigned error;\\ (ii) Mean signed error; \\ (iii) RMSE\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 58.62 $\pm$ 43.12 $\mu$m \citep{Hussain2015}. 26.65 $\pm$ 13.27 $\mu$m \citep{Antony2014}.\\  22.22 $\pm$ 5.99 $\mu$m \citep{Miri2017}.\\ (ii) 6.61 $\pm$ 18.59 $\mu$m \citep{Antony2014}. -0.30 $\pm$ 12.44 $\mu$m \citep{Miri2017}.\\ (iii) 17.99 $\pm$ 8.15 $\mu$m \citep{Antony2014}. 11.62 $\pm$ 4.63 $\mu$m \citep{Miri2017}\end{tabular} \\ \hline
Optic Cup &
  \begin{tabular}[c]{@{}l@{}}(i) Correlation with ground truth;   \\ (ii) Error compared with ground truth;\\ (iii) Mean unsigned error;\\ (iv) Dice similarity coefficient\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 0.80 \citep{Boyer2006}\\ (ii) 3.4 pixels (normal) and 3.6 pixels (glaucoma) \citep{Paul2015}\\ (iii) 0.009 mm \citep{Lee2009}. 0.038 mm \citep{Lee2010}\\ (iv) 0.85 $\pm$ 0.06 \citep{Lee2010}\end{tabular} \\ \hline
CDR &
  \begin{tabular}[c]{@{}l@{}}(i) Error compared with ground truth;\\ (ii) Sensitivity;\\ (iii) Specificity;\\ (iv) Accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 0.045 $\pm$ 0.033 \citep{Wu2015} \\ (ii) 86.2 $\pm$ 7.1\% \citep{Khalil2018}\\ (iii) 86.2 $\pm$ 9.8\% \citep{Khalil2018}\\ (iv) 85.5 $\pm$ 5.2\% \citep{Khalil2018}\end{tabular} \\ \hline
ILM &
  \begin{tabular}[c]{@{}l@{}}(i) Mean unsigned error; \\ (ii) Mean Dice coefficient;\\ (iii) Error compared with ground truth;\\ (iv) Mean Euclidean distance error\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 5.38 $\pm$ 4.23 $\mu$m \citep{Yu2018}.\\ (ii) 0.97 \citep{Heisler2020}.\\ (iii) 4.80 $\mu$m \citep{Gawlik2018}\\ (iv) 7.08 $\pm$ 3.7 pixels \citep{Ramzan2018a}. 7.03 $\pm$ 3.72 pixels\end{tabular} \\ \hline
LC &
  \begin{tabular}[c]{@{}l@{}}(i) Failure rate;  \\ (ii) Accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 0 in 73.7\% of the scans \citep{Belghith2015} \\ (ii) 90.6\% \citep{Mao2019}\end{tabular} \\ \hline
ONH surface depth &
  (i) Error compared with ground truth &
  (i)  0.7 $\pm$ 1.0 \% \citep{Ko2016}. \\ \hline
\end{tabular}%
}

\end{table*}

==> LC OCT segmentation (arxiv)/region_based.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h]
\centering
\caption{Results from the region based segmentation}
\label{tab:region based}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllc}
\hline
%\multicolumn{4}{c}{Region based segmentation} \\ \hline
\multicolumn{1}{c}{Outcome} &
  \multicolumn{1}{c}{Metrics} &
  \multicolumn{2}{c}{Results} \\ \hline
RNFL + prelamina &
  \begin{tabular}[c]{@{}l@{}}(i) Dice coefficient;\\ (ii) Sensitivity;\\ (iii) Specificity;\\ (iv) Accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 0.82 $\pm$ 0.05 \citep{Devalla2018a}. 0.92 $\pm$ 0.05 for healthy \\ and 0.92 $\pm$ 0.03 for glaucoma \citep{Devalla2018}. \\ (ii) 0.89 $\pm$ 0.04 \citep{Devalla2018a}\\ (iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.\\ (iv) 0.93 $\pm$ 0.02 \citep{Devalla2018a}\end{tabular} &
  \multirow{15}{*}{\begin{tabular}[c]{@{}c@{}}  Mean for all tissues:\\ (ii) 0.94 $\pm$ 0.02 (Spectralis), \\ 0.93 $\pm$ 0.02 (Cirrus) and \\0.93 $\pm$ 0.02 (RTVue) \citep{Devalla2020}.\\ (iii) 0.99 for Spectralis, Cirrus \\ and RTVue \citep{Devalla2020}.\end{tabular}} \\ \cline{1-3}
RPE &
  \begin{tabular}[c]{@{}l@{}}(i) Dice coefficient \\ (ii) Sensitivity;\\ (iii) Specificity;\\ (iv) Accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 0.84 $\pm$ 0.02  \citep{Devalla2018a}. 0.83 $\pm$ 0.04 for healthy  \\ and 0.84 $\pm$ 0.03 for glaucoma \citep{Devalla2018}.\\ (ii) 0.90 $\pm$ 0.03 \citep{Devalla2018a}\\ (iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.\\ (iv) 0.93 $\pm$ 0.02 \citep{Devalla2018a}\end{tabular} &
   \\ \cline{1-3}
Other retinal layers &
  \begin{tabular}[c]{@{}l@{}}(i) Dice coefficient\\ (ii) Sensitivity;\\ (iii) Specificity;\\ (iv) Accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 0.86 $\pm$ 0.03  \citep{Devalla2018a}. 0.95 $\pm$ 0.01 for healthy \\ and 0.96 $\pm$ 0.03 for glaucoma \citep{Devalla2018}.\\ (ii) 0.98 $\pm$ 0.02 \citep{Devalla2018a}\\ (iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.\\ (iv) 0.98 $\pm$ 0.01 \citep{Devalla2018a}\end{tabular} &
   \\ \cline{1-3}
Choroid &
  \begin{tabular}[c]{@{}l@{}}(i) Dice coefficient\\ (ii) Sensitivity;\\ (iii) Specificity;\\ (iv) Accuracy\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(i) 0.85 $\pm$ 0.02 \citep{Devalla2018a}. 0.90 $\pm$ 0.03 for healthy \\ and 0.91 $\pm$ 0.05 for glaucoma \citep{Devalla2018}.\\ (ii) 0.91 $\pm$ 0.02 \citep{Devalla2018a}\\ (iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.\\ (iv) 0.93 $\pm$ 0.01 \citep{Devalla2018a}\end{tabular} &
   \\ \hline
\end{tabular}%
}


\end{table*}

==> Results_Table.tex <==
\def\arraystretch{1.5}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}

\begin{scriptsize}
\begin{landscape}
%\begin{table*}
\begin{longtable}{C{2cm}C{3cm}C{3.5cm}C{15cm}}
\caption{Results}\\ \hline
%\begin{tabular}{p{20mm}p{30mm}p{35mm}p{150mm}}

%\hline

Segmentation            & Outcome              & Metrics & Results \\ \hline
\multirow{5}{*}{Boundary based}  & \ac{BMO} 
& (i) Correlation with ground truth; 
(ii) Error compared with ground truth; 
(iii) Mean unsigned error; 
(iv) Mean signed error;
(v) Dice similarity coefficient;
(vi) Failure rate;
(vii) Mean average precision
&    
(i) 0.93 \citep{Boyer2006}; 
(ii) 32.03 $\pm$ 58.68 $\mu$m \citep{Mokhtari2017}. 12.4 $\pm$ 12.1 pixels \citep{Fu2015}. 2.8 pixels (normal) and 3.1 pixels (glaucoma) \citep{Paul2015}. 54.18 $\pm$ 53.74 $\mu$m \citep{Hussain2015}. 60.00 $\pm$ 42.00 $\mu$m \citep{Wu2015}. 49.28 $\pm$ 16.78 $\mu$m \citep{Miri2017}. 42.38 $\pm$ 18.33 $\mu$m \citep{Chen2019}.
(iii) 61.86 $\pm$ 61.97 $\mu$m (x axis) and 12.40 $\pm$ 11.24 $\mu$m (z axis) \citep{Yadav2018}. 49.53 $\pm$ 30.41 $\mu$m (x axis) and 31.58 $\pm$ 21.06 $\mu$m (z axis) \citep{Antony2014}. 37.98 $\pm$ 14.91 $\mu$m (x axis) and 22.28 $\pm$ 8.58 $\mu$m (z axis) \citep{Miri2017}. 9.80 $\pm$ 31.90 $\mu$m \citep{Skander2020}. 0.023 mm \citep{Lee2009}. 0.026 mm \citep{Lee2010}
(iv)  −7.69 $\pm$ 87.27 $\mu$m (x axis) and −1.41 $\pm$ 16.69 $\mu$m (z axis) \citep{Yadav2018}. 26.49 $\pm$ 40.22 $\mu$m (x axis) and 25.45 $m$ 14.37 $\mu$m (z axis) \citep{Antony2014}. -9.49 $\pm$ 24.58 $\mu$m (x axis) and 8.33 $\pm$ 17.72 $\mu$m (z axis) \citep{Miri2017}.
(v) 0.925 $\pm$ 0.030 \citep{Yu2018}. 0.959 $\pm$ 0.032 \citep{Skander2020}. 0.65 $\pm$ 0.14 \citep{Lee2010}.
(vi) 0 in 92.5\% of the scans \citep{Belghith2014}
(vii) 0.8547 for glaucoma and 0.9567 for control subjects \citep{Heisler2020}.
\\ \cline{2-4} 
                                & \ac{BMO-MRW}              
&  (i) Mean unsigned error;
(ii) Mean signed error; 
(iii) RMSE
&  (i) 58.62 $\pm$ 43.12 $\mu$m \citep{Hussain2015}. 26.65 $\pm$ 13.27 $\mu$m \citep{Antony2014}. 22.22 $\pm$ 5.99 $\mu$m \citep{Miri2017}.
(ii) 6.61 $\pm$ 18.59 $\mu$m \citep{Antony2014}. -0.30 $\pm$ 12.44 $\mu$m \citep{Miri2017}.
(iii) 17.99 $\pm$ 8.15 $\mu$m \citep{Antony2014}. 11.62 $\pm$ 4.63 $\mu$m \citep{Miri2017} \\ \cline{2-4} 
                                & Optic cup            
&  (i) Correlation with ground truth;   
(ii) Error compared with ground truth;
(iii) Mean unsigned error;
(iv) Dice similarity coefficient
&  (i) 0.80 \citep{Boyer2006}
(ii) 3.4 pixels (normal) and 3.6 pixels (glaucoma) \citep{Paul2015}
(iii) 0.009 mm \citep{Lee2009}. 0.038 mm \citep{Lee2010}
(iv) 0.85 $\pm$ 0.06 \citep{Lee2010} \\ \cline{2-4} 
                                & \ac{CDR}  
& (i) Error compared with ground truth;
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
& (i) 0.045 $\pm$ 0.033 \citep{Wu2015} 
(ii) 86.2 $\pm$ 7.1\% \citep{Khalil2018}
(iii) 86.2 $\pm$ 9.8\% \citep{Khalil2018}
(iv) 85.5 $\pm$ 5.2\% \citep{Khalil2018} \\ \cline{2-4} 
                                & \ac{ILM}   
&  (i) Mean unsigned error; 
(ii) Mean Dice coefficient;
(iii) Error compared with ground truth;
(iv) Mean Euclidean distance error
&   (i) 5.38 $\pm$ 4.23 $\mu$m \citep{Yu2018}.
(ii) 0.97 \citep{Heisler2020}.
(iii) 4.80 $\mu$m \citep{Gawlik2018}
(iv) 7.08 $\pm$ 3.7 pixels \citep{Ramzan2018a}. 7.03 $\pm$ 3.72 pixels \citep{Ramzan2018b} \\ \cline{2-4} 
                                & \ac{LC}                   
&  (i) Failure rate;  
(ii) Accuracy
&  (i) 0 in 73.7\% of the scans \citep{Belghith2015} 
(ii) 90.6\% \citep{Mao2019}      \\ \cline{2-4} 
                                & \ac{ONH} surface depth                
&   (i) Error compared with ground truth     
&    (i)  0.7 $\pm$ 1.0 \% \citep{Ko2016}.   \\ \hline
\multirow{6}{*}{Region based}   & \ac{RNFL} + prelamina     
& (i) Dice coefficient;
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
& (i) 0.82 $\pm$ 0.05 \citep{Devalla2018a}. 0.92 $\pm$ 0.05 for healthy and 0.92 $\pm$ 0.03 for glaucoma \citep{Devalla2018}. 
(ii) 0.89 $\pm$ 0.04 \citep{Devalla2018a}
(iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.
(iv) 0.93 $\pm$ 0.02 \citep{Devalla2018a} \\ \cline{2-4} 
                                & \ac{RPE}                  
& (i) Dice coefficient 
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
& (i) 0.84 $\pm$ 0.02  \citep{Devalla2018a}. 0.83 $\pm$ 0.04 for healthy and 0.84 $\pm$ 0.03 for glaucoma \citep{Devalla2018}.
(ii) 0.90 $\pm$ 0.03 \citep{Devalla2018a}
(iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.
(iv) 0.93 $\pm$ 0.02 \citep{Devalla2018a}
 \\ \cline{2-4} 
                                & Other retinal layers 
& (i) Dice coefficient
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
&  (i) 0.86 $\pm$ 0.03  \citep{Devalla2018a}. 0.95 $\pm$ 0.01 for healthy and 0.96 $\pm$ 0.03 for glaucoma \citep{Devalla2018}.
(ii) 0.98 $\pm$ 0.02 \citep{Devalla2018a}
(iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.
(iv) 0.98 $\pm$ 0.01 \citep{Devalla2018a}
 \\ \cline{2-4} 
                                & Choroid              
& (i) Dice coefficient
(ii) Sensitivity;
(iii) Specificity;
(iv) Accuracy
&  (i) 0.85 $\pm$ 0.02 \citep{Devalla2018a}. 0.90 $\pm$ 0.03 for healthy and 0.91 $\pm$ 0.05 for glaucoma \citep{Devalla2018}.
(ii) 0.91 $\pm$ 0.02 \citep{Devalla2018a}
(iii) 0.99 \citep{Devalla2018a}. 0.99 \citep{Devalla2018}.
(iv) 0.93 $\pm$ 0.01 \citep{Devalla2018a}        \\ \hline 

\label{tab:results}
%\end{tabular}
\end{longtable}
%\end{table*}
\end{landscape}
\end{scriptsize}
